Unbiased Statistical Estimation and Valid Confidence Intervals Under Differential Privacy

We present a method for producing unbiased parameter estimates and valid confidence intervals under the constraints of differential privacy, a formal framework for limiting individual information leakage from sensitive data. Prior work in this area is limited in that it is tailored to calculating confidence intervals for specific statistical procedures, such as mean estimation or simple linear regression. While other recent work can produce confidence intervals for more general sets of procedures, they either yield only approximately unbiased estimates, are designed for one-dimensional outputs, or assume significant user knowledge about the data-generating distribution. Our method induces distributions of mean and covariance estimates via the bag of little bootstraps (BLB) and uses them to privately estimate the parameters' sampling distribution via a generalized version of the CoinPress estimation algorithm. If the user can bound the parameters of the BLB-induced parameters and provide heavier-tailed families, the algorithm produces unbiased parameter estimates and valid confidence intervals which hold with arbitrarily high probability. These results hold in high dimensions and for any estimation procedure which behaves nicely under the bootstrap.

==> parameter_estimation.tex <==
\section{Final Parameter Estimation via Post-Processing}
\label{sec:parameter_estimation}

Now that we have a way of privately estimating the means of the BLB-induced distributions, 
$\hat{\theta}^{BLB}$ and $\hat{\Sigma}^{BLB}$,
we can move to lines~\ref{ln:gvdp:prec_weight_cov}, \ref{ln:gvdp:prec_weight_mean}, and~\ref{ln:gvdp:get_cis} of 
Algorithm~\ref{alg:gvdp}, where we use the private estimates we get from CoinPress to produce our final parameter estimates
and confidence intervals.

We start by noting a theorem that will be used throughout this section, whose proof can 
be found in Section~\ref*{appendix:subsection:proof:precision_weighting}.
This is the multivariate version of the inverse-variance weighting argument commonly 
found in the meta-analysis literature, which gives the optimal (i.e.\ minimum covariance) way to combine a 
set of unbiased estimators.

\begin{theorem}
	\label{theorem:precision_weighting}
	For a parameter $\tau$, say we are given a series of independent estimates $\{ \hat{\tau}_m \}_{m \in [t]}$
	such that $\E \left( \hat{\tau}_m \right) = \tau$ and $Cov \left( \hat{\tau}_m \right) = S_m$
	for some positive definite (PD) $S_m$. Note that this is slightly stronger than the PSD assumption we have been making.
	Then the minimum covariance unbiased linear weighting 
	of the $\{ \hat{\tau}_m \}_{m \in [t]}$ is given by 
	\[ \hat{\tau} = \left( \Sigma_{m=1}^{t} S_m^{-1} \right)^{-1} \left( \Sigma_{m = 1}^{t} S_m^{-1} \hat{\tau}_m \right), \]
	which has 
	$\E \left( \hat{\tau} \right) = \tau$
	and 
	$Cov \left( \hat{\tau} \right) = \left( \Sigma_{m=1}^{t} S_m^{-1} \right)^{-1}$.

	Specifically, by ``minimum covariance'' we mean that any other unbiased linear weighting $\hat{\tau}'$ of the $\hat{\tau}_m$ will have 
	$Cov \left( \hat{\tau} \right) \preceq Cov \left( \hat{\tau}' \right)$. 
\end{theorem}

% \subsection{Privately estimating $\hat{\Sigma}$}
% \label{subsec:estimating_Sigma}

We now explore how to aggregate our $\{\hat{\Sigma}^{BLB}_i\}_{i \in [k]}$ to get a differentially private estimate of 
$\hat{\Sigma}$. 
Here, we consider only the case where we estimate only the diagonal of $\hat{\Sigma}$, as this is 
sufficient for confidence intervals. 
Our methods generalize to estimating the full $\hat{\Sigma}$, which can be used for more general confidence sets.
Details can be found in Section~\ref*{appendix:section:estimating_full_sigma_hat}.

% We consider two separate cases; one where we estimate only the diagonal of $\hat{\Sigma}^{BLB}$, which is 
% sufficient if we want confidence intervals,
% and one where we estimate the full matrix, which we use if we want a more general confidence set.

\subsection{Privately estimating diagonal of $\hat{\Sigma}$}
\label{subsec:estimating_diagonal_Sigma_hat}

We first consider the case where we care only about the diagonal of $\hat{\Sigma}^{BLB}$;
that is, we don't care about the covariance structure of our parameters.
Thus, without loss of generality, we write $\hat{\Sigma}^{BLB}_i = \hat{V}_i I_d$ where $\hat{v}_{i,j}$ is the $j^{th}$ element of $\hat{V}_i$.
Though $\hat{V}$ is a random variable, we abuse notation in the typical way and also let 
$\hat{V} = \frac{1}{k} \sum_{i=1}^{k}\hat{V}_i$.
Because we are assuming the off-diagonal elements of $\Sigma$ are 0, estimating $\Sigma$ reduces to 
estimating $V$. 

We assume the user provides initial conditions such that  
Assumptions~\ref{assump:user_heavier_tailed}, 
\ref{assump:initial_parameter_bounds}, and
\ref{assump:initial_covariance_bounds}, 
hold and appeal to Algorithm~\ref{alg:hd_mean_est},
substituting $\hat{V}_i$ for the general $\hat{\mu}_i$ from those statements. 
This yields the following result, which we prove in section~\ref*{appendix:subsection:proof:estimating_diagonal_of_sigma_hat}.

\begin{theorem}
	\label{theorem:diagonal_sigma-loewner_ub}
	Applying Algorithm~\ref{alg:hd_mean_est} to $\hat{M} = ( \hat{V}_1, \hdots, \hat{V}_k )$
	yields $\{ \tilde{V}_m, \vec{\sigma}^2_m \}_{m \in [t]}$.

	We combine these into an estimator
	\begin{equation}
		\label{eq:diag_cov_est-inverse_cov_weighting}
		\tilde{V} = \frac{ \sum_{m=1}^{t} \tilde{V}_m / \vec{\sigma}_m^2 }{ \sum_{m=1}^{t} 1 / \vec{\sigma}_m^2 }.
	\end{equation}
	Define $\Phi^{-1}$ as the quantile function of the standard Gaussian and let 
	\begin{equation}
		\label{eq:diag_cov_est-noise_ub}
		\vec{\gamma} = \frac{1}{ \sqrt{ \sum_{m=1}^{t} 1/\vec{\sigma}_m^2 } } \Phi^{-1} \left( 1 - \beta^{ub}/d \right)
	\end{equation}
	for arbitrary $\beta^{ub} \in (0,1)$. 
	Then, for  
	$\tilde{\Sigma} = (\tilde{V} + \vec{\gamma}) I_d$
	we have
	\[ \Pr \left( \forall j \in [d]: \hat{\Sigma}_{j,j} \leq \tilde{\Sigma}_{j,j} \right) \geq 1 - \beta^{\tilde{V}} - \beta^{ub}. \]
\end{theorem}

In order to have consistent notation between the diagonal and full $\hat{\Sigma}$ settings, 
we will refer to $\beta^{\tilde{V}}$ as $\beta^{\tilde{\Sigma}}$
and refer to $\hat{\Sigma}$ as if it were diagonal such that
if $\forall j \in [d]: \hat{\Sigma}_{j,j} \leq \tilde{\Sigma}_{j,j}$, then 
$\hat{\Sigma} \preceq \tilde{\Sigma}$.

% \subsection{Estimating full $\hat{\Sigma}$}
% \label{subsec:estimating_full_Sigma_hat}
% In the case where we care about the covariance structure of our parameters, we instead estimate 
% the entire $\hat{\Sigma}^{BLB}$ matrix. 
% We start by creating a flattened upper triangular of each $\hat{\Sigma}^{BLB}_i$, which we call 
% $\hat{S}^{\flat}_i \in \R^{\frac{d(d+1)}{2}}$.
% Our analysis then proceeds much like it did in 
% Section~\ref{subsec:estimating_diagonal_Sigma_hat}.
% The primary difference is that we no longer treat upper bounding the diagonal of 
% $\hat{\Sigma}^{BLB}$ as sufficient for valid confidence intervals. Instead, 
% we need a full L{\"o}wner upper bound on $\hat{\Sigma}^{BLB}$.
% Again, we assume the user provides initial conditions such that 
% Assumptions~\ref{assump:user_heavier_tailed},
% \ref{assump:initial_parameter_bounds}, and
% \ref{assump:initial_covariance_bounds} 
% hold and appeal to Algorithm~\ref{alg:hd_mean_est}.
% We also use Algorithm~\ref*{appendix:alg:high_prob_upper_bound} (HPUB),
% which produces a high-probability upper bound on a specified random variable. 

% \begin{theorem}
% 	\label{theorem:full_sigma-loewner_ub}
% 	Applying Algorithm~\ref{alg:hd_mean_est} to $\hat{M} = ( \hat{S}^{\flat}_1, \hdots, \hat{S}^{\flat}_k )$
% 	yields $\{ \tilde{S}^{\flat}_m, \vec{\sigma}^2_m \}_{m \in [t]}$.

% 	We combine these into a single estimate
% 	\begin{equation*}
% 		\label{eq:full_cov_est-inverse_cov_weighting}
% 		\tilde{S}^{\flat} = \frac{ \sum_{m=1}^{t} \tilde{S}^{\flat}_m / \vec{\sigma}_m^2 }{ \sum_{m=1}^{t} 1 / \vec{\sigma}_m^2 }
% 	\end{equation*}	 
% 	and unflatten it back to a matrix $\tilde{S} \in \R^{d \times d}$.
% 	Let
% 	\begin{equation*}
% 		\label{eq:full_cov_est-noise_ub}
% 		\gamma = HPUB \left( \Vert \sigma_M^2 \Vert_2, \beta^{ub} \right)
% 	\end{equation*} 
% 	where $\sigma_M^2 \in \R^{d \times d}$ 
% 	is the unflattened version of $\frac{1}{ \sum_{m=1}^{t} 1/\vec{\sigma}_m^2 }$.

% 	Then, for  
% 	$\tilde{\Sigma} = \tilde{S} + \gamma I_d$
% 	we have
% 	$\Pr \left( \hat{\Sigma} \preceq \tilde{\Sigma} \right) \geq 1 - \beta^{\tilde{S}} - \beta^{ub}$.
% \end{theorem}
% See Section~\ref*{appendix:subsection:proof:estimating_full_sigma_hat} for a proof.
% As before, we refer to $\beta^{\tilde{S}}$ as 
% $\beta^{\tilde{\Sigma}}$ in the interest of more consistent notation.

\subsection{Privately estimating $\hat{\theta}$}
\label{subsec:estimating_theta}

To privately estimate $\hat{\theta}$, we again use Algorithm~\ref{alg:hd_mean_est}, 
substituting $\hat{\theta}_i$ for $\hat{\mu}_i$ in the general statement.
We again assume the user provides initial conditions such that 
Assumptions~\ref{assump:user_heavier_tailed} and \ref{assump:initial_parameter_bounds}
hold. 

We could assume that the user provides bounds that respect Assumption~\ref{assump:initial_covariance_bounds}, 
but we have another option available to us which will often give much tighter estimates; 
relating the private estimate $\tilde{\Sigma}$ to the 
covariance of the $\{ \hat{\theta}_i^{BLB} \}_{i \in [k]}$.

Although we are scaling up our subsets to the original data size within the BLB to get correct overall covariance 
estimates, this does not imply that the covariance of our $\{ \hat{\theta}_i^{BLB} \}_{i \in [k]}$ is 
appropriately scaled. In fact, this covariance will often be roughly the same as if $\hat{\theta}$ were simply 
run on subsets of size $\frac{n}{k}$. So, the covariance of the $\{ \hat{\theta}_i^{BLB} \}_{i \in [k]}$
should be roughly $\frac{r(n/k)}{r(n)} \hat{\Sigma}$, where $r$ is the convergence rate of the estimator 
in question. For example, the covariance of OLS coefficients decays with $\frac{1}{n}$, so if $\hat{\theta}$
represents OLS estimation we would say the covariance is $\frac{1/(n/k)}{1/n} \Sigma = k \hat{\Sigma}$. 
We upper bound this with $k \tilde{\Sigma}$.
% Under Assumption~\ref{assump:blb_approx}, $k \tilde{\Sigma}$ will be a 
% L{\"o}wner upper bound on $k \hat{\Sigma}$ with probability $1 - \beta^{\tilde{\Sigma}}$
% provided we privately estimate the entire covariance matrix as in 
% Section~\ref{subsec:estimating_full_Sigma_hat}. 
Under Assumption~\ref{assump:blb_approx}, we 
have a $1-\beta^{\tilde{\Sigma}}$ probability guarantee that $k \tilde{\Sigma}$ will 
upper bound the empirical variance in each dimension.

\begin{theorem}
	\label{theorem:theta_est}
	Applying Algorithm~\ref{alg:hd_mean_est} to $\hat{M} = ( \hat{\theta}_1, \hdots, \hat{\theta}_k )$
	yields $\{ \tilde{H}_m, \vec{\sigma}^2_m \}_{m \in [t]}$.

    We then construct a combined estimator $\tilde{\theta}$ where 
	\begin{equation}
		\label{eq:theta_est-inverse_cov_weighting}
		\tilde{\theta} = \frac{ \sum_{m=1}^{t} \tilde{H}_m / \vec{\sigma}_m^2 }{ \sum_{m=1}^{t} 1 / \vec{\sigma}_m^2 }.
	\end{equation}
    This new estimator has covariance $\Sigma_{\tilde{\theta}} = \frac{1}{ \sum_{m=1}^{t} 1/\vec{\sigma}_m^2 }I_d$.

    In particular, we say that 
    $\Pr \left( \tilde{\theta} \sim N \left( \theta, \Sigma_{\tilde{\theta}} \right) \right) \geq 1 - \beta^{\tilde{\Sigma}} - \beta^{ub} - \beta^{\tilde{\theta}}$.
\end{theorem}

See Section~\ref*{appendix:subsection:proof:privately_estimating_theta_hat} for a proof.

% \cnote{need to make sure I can actually justify using $\theta$ rather than, say, $\hat{\theta}^{BLB}$ above}

\subsection{Confidence Intervals}
\label{subsec:confidence_intervals}
We now have estimates of the mean and covariance of $\hat{\theta}$; $\tilde{\theta}$ and $\tilde{\Sigma}$ respectively,
such that $\tilde{\theta} \sim N\left( \hat{\theta}, \Sigma_{\tilde{\theta}} \right)$ and $\hat{\Sigma} \preceq \tilde{\Sigma}$ 
with probability $1 - \beta^{\tilde{\Sigma}} - \beta^{ub} - \beta^{\tilde{\theta}}$, 
as well as a distribution $Q_{\tilde{\theta}}$ we assume to be heavier tailed than that of $\hat{\theta}$. 
We can represent our approximation of the sampling distribution as the compound distribution
\begin{equation}
	\label{eq:compound_distribution}
	Q_{\tilde{\theta}} \left( \hat{\theta} + N \left(0, \Sigma_{\tilde{\theta}} \right), \tilde{\Sigma} \right),
\end{equation}
where we interpret $\hat{\theta}$ and $\tilde{\Sigma}$ as realizations of their random variables.  

We appeal to Algorithm~\ref*{appendix:alg:ci_simulation}, which in turn
uses Algorithm~\ref*{appendix:alg:high_prob_upper_bound} to get an upper/lower bounds on quantiles of a random variable.
This yields two different notions of confidence intervals; one for which the confidence interval is valid with 
high probability, and one which is valid with probability 1. See Section~\ref*{appendix:subsection:general_ci_high_prob} 
for proofs.

\begin{theorem}[General confidence intervals (valid with high probability)]
	\label{theorem:general_ci_high_prob}
	We apply Algorithm~\ref*{appendix:alg:ci_simulation} to each dimension of $Q_{\tilde{\theta}}$ at levels $\{\alpha_j\}_{j \in [d]}$ and get 
	$\{ (ci^l_j, ci^u_j) \}_{j \in [d]}$. Then,
    with probability $1 - \beta^{\tilde{\Sigma}} - \beta^{ub} - \beta^{\tilde{\theta}}$, 
    \[ \forall j \in [d]: \Pr \left( \hat{\theta}_j \in \left( ci^l_j, ci^u_j \right) \right) \geq 1 - \alpha_j. \]
\end{theorem}

\begin{corollary}[General confidence intervals (valid with probability 1)]
	\label{corollary:general_ci_prob_1}
    For all $j \in [d]$, let $\alpha'_j = \alpha_j - \beta^{\tilde{\Sigma}} - \beta^{ub} - \beta^{\tilde{\theta}}$ for some $\{\alpha_j\}_{j \in [d]}$. 
	Then, provided that $\forall j \in [d]: \alpha'_j > 0$, we apply Algorithm~\ref*{appendix:alg:ci_simulation} to each dimension of $Q_{\tilde{\theta}}$ 
	at levels $\{\alpha'_j\}_{j \in [d]}$ and get 
	$\{ (ci^l_j, ci^u_j) \}_{j \in [d]}$. Then,
    \[ \forall j \in [d]: \Pr \left( \hat{\theta}_j \in \left( ci^l_j, ci^u_j \right) \right) \geq 1 - \alpha_j. \]
\end{corollary}

Note that although we give these results based on a general $Q_{\tilde{\theta}}$, the compound distribution behaves much more nicely for 
many distributions. 
Most notable is that if $Q_{\tilde{\theta}}$ is multivariate Gaussian, the resulting compound distribution is 
$N \left(\tilde{\theta}, \tilde{\Sigma} + \Sigma_{\tilde{\theta}} \right)$. 
In this case, we note that 
$\forall j \in [d]: \tilde{\theta}_j \sim N \left( \hat{\theta}_j, \tilde{\Sigma}_{j,j} + \Sigma_{\tilde{\theta}_{j,j}} \right)$,
and so we can calculate confidence intervals directly from the CDF of the univariate Gaussian.

Although we focus on confidence intervals here, these results can be generalized to confidence sets, provided 
that the full private covariance is estimated as in Theorem~\ref*{appendix:theorem:full_sigma-loewner_ub} and you 
are able to integrate the multivariate compound distribution in Equation~\ref{eq:compound_distribution}.
